Learning Field Reconstruction from Incomplete Data by Globally Correcting Local Estimates

Reconstructing physical fields from training samples that are always incomplete requires learning spatial structure from fragmented observations. Existing context--query work establishes how held-out observations provide valid training targets, but this does not make the complete-field distribution identifiable when every training field is incomplete. With finite data, weak evidence of sharp transitions and localized variations can further favor averaged predictions that attenuate local detail. A structural prior is therefore needed to favor plausible completions; local spatial relationships offer one grounded in the observations. We propose a locally constructed, globally revisable estimator that explicitly learns local field estimates and subsequently corrects them using full-domain observations. A shared coordinate-conditioned predictor learns from incomplete patches, allowing relatively well-observed neighborhoods to provide direct supervision of local structure. Its overlapping predictions are reconciled into an observation-conditioned consensus field. A full-domain estimator retains the original observations and learns a residual correction around this frozen field estimate, allowing locally constructed structure to be revised by broader evidence. The local estimate serves as both an explicit input, accompanied by its discrepancies with the observations, and a prediction starting point that the global model can revise. On three real-world ocean datasets with authentic observation gaps, our estimator achieves the lowest MSE and highest PSNR on withheld source-supported values, reducing MSE by 28.9%--34.5% against the strongest external baseline.

==> visualizations/detail_horizontal_style.tex <==
\definecolor{detailOrange}{RGB}{240,154,0}
\def\DetailWidth{69.85}
\def\DetailHeight{38.7}
\def\DetailPanelSize{21.3}
\def\DetailLeftX{0.35}
\def\DetailReferenceX{24.275}
\def\DetailRightX{48.2}
\def\DetailTop{9.2}
\def\DetailBarX{20.425}
\def\DetailBarWidth{29}
\tikzset{detail outline/.style={draw=detailOrange,line width=0.5pt,line cap=butt,line join=miter}}
\newcommand{\DetailHorizontalLabels}[1]{%
  \node[anchor=base,font=\VisualizationLabelFont] at ({\DetailLeftX+\DetailPanelSize/2},3.35) {#1};
  \node[anchor=base,font=\VisualizationLabelFont] at ({\DetailReferenceX+\DetailPanelSize/2},3.35) {Reference};
  \node[anchor=base,font=\VisualizationLabelFont] at ({\DetailRightX+\DetailPanelSize/2},3.35) {Ours};
  \node[anchor=base,font=\VisualizationLabelFont] at ({\DetailLeftX+\DetailPanelSize/2},6.85) {Zoom};
  \node[anchor=base,font=\VisualizationLabelFont] at ({\DetailReferenceX+\DetailPanelSize/2},6.85) {Full field};
  \node[anchor=base,font=\VisualizationLabelFont] at ({\DetailRightX+\DetailPanelSize/2},6.85) {Zoom};
}
\newcommand{\DetailHorizontalAnnotations}[4]{%
  \draw[detail outline] (\DetailLeftX,\DetailTop) rectangle ++(\DetailPanelSize,\DetailPanelSize);
  \draw[detail outline] (\DetailRightX,\DetailTop) rectangle ++(\DetailPanelSize,\DetailPanelSize);
  \draw[detail outline] ({\DetailReferenceX+\DetailPanelSize*#1/64},{\DetailTop+\DetailPanelSize*#3/64})
    rectangle ({\DetailReferenceX+\DetailPanelSize*#2/64},{\DetailTop+\DetailPanelSize*#4/64});
  \draw[detail outline] ({\DetailReferenceX+\DetailPanelSize*#1/64},{\DetailTop+\DetailPanelSize*(#3+#4)/128})
    -- ({\DetailLeftX+\DetailPanelSize},{\DetailTop+\DetailPanelSize/2});
  \draw[detail outline] ({\DetailReferenceX+\DetailPanelSize*#2/64},{\DetailTop+\DetailPanelSize*(#3+#4)/128})
    -- (\DetailRightX,{\DetailTop+\DetailPanelSize/2});
}


==> visualizations/figure1_colors.tex <==
\definecolor{oceanonefield0}{rgb}{0.267004,0.004874,0.329415}
\definecolor{oceanonefield1}{rgb}{0.269944,0.014625,0.341379}
\definecolor{oceanonefield2}{rgb}{0.272594,0.025563,0.353093}
\definecolor{oceanonefield3}{rgb}{0.274952,0.037752,0.364543}
\definecolor{oceanonefield4}{rgb}{0.277018,0.050344,0.375715}
\definecolor{oceanonefield5}{rgb}{0.278791,0.062145,0.386592}
\definecolor{oceanonefield6}{rgb}{0.280267,0.073417,0.397163}
\definecolor{oceanonefield7}{rgb}{0.281446,0.084320,0.407414}
\definecolor{oceanonefield8}{rgb}{0.282327,0.094955,0.417331}
\definecolor{oceanonefield9}{rgb}{0.282910,0.105393,0.426902}
\definecolor{oceanonefield10}{rgb}{0.283197,0.115680,0.436115}
\definecolor{oceanonefield11}{rgb}{0.283187,0.125848,0.444960}
\definecolor{oceanonefield12}{rgb}{0.282884,0.135920,0.453427}
\definecolor{oceanonefield13}{rgb}{0.282290,0.145912,0.461510}
\definecolor{oceanonefield14}{rgb}{0.281412,0.155834,0.469201}
\definecolor{oceanonefield15}{rgb}{0.280255,0.165693,0.476498}
\definecolor{oceanonefield16}{rgb}{0.278826,0.175490,0.483397}
\definecolor{oceanonefield17}{rgb}{0.277134,0.185228,0.489898}
\definecolor{oceanonefield18}{rgb}{0.275191,0.194905,0.496005}
\definecolor{oceanonefield19}{rgb}{0.273006,0.204520,0.501721}
\definecolor{oceanonefield20}{rgb}{0.270595,0.214069,0.507052}
\definecolor{oceanonefield21}{rgb}{0.267968,0.223549,0.512008}
\definecolor{oceanonefield22}{rgb}{0.265145,0.232956,0.516599}
\definecolor{oceanonefield23}{rgb}{0.262138,0.242286,0.520837}
\definecolor{oceanonefield24}{rgb}{0.258965,0.251537,0.524736}
\definecolor{oceanonefield25}{rgb}{0.255645,0.260703,0.528312}
\definecolor{oceanonefield26}{rgb}{0.252194,0.269783,0.531579}
\definecolor{oceanonefield27}{rgb}{0.248629,0.278775,0.534556}
\definecolor{oceanonefield28}{rgb}{0.244972,0.287675,0.537260}
\definecolor{oceanonefield29}{rgb}{0.241237,0.296485,0.539709}
\definecolor{oceanonefield30}{rgb}{0.237441,0.305202,0.541921}
\definecolor{oceanonefield31}{rgb}{0.233603,0.313828,0.543914}
\definecolor{oceanonefield32}{rgb}{0.229739,0.322361,0.545706}
\definecolor{oceanonefield33}{rgb}{0.225863,0.330805,0.547314}
\definecolor{oceanonefield34}{rgb}{0.221989,0.339161,0.548752}
\definecolor{oceanonefield35}{rgb}{0.218130,0.347432,0.550038}
\definecolor{oceanonefield36}{rgb}{0.214298,0.355619,0.551184}
\definecolor{oceanonefield37}{rgb}{0.210503,0.363727,0.552206}
\definecolor{oceanonefield38}{rgb}{0.206756,0.371758,0.553117}
\definecolor{oceanonefield39}{rgb}{0.203063,0.379716,0.553925}
\definecolor{oceanonefield40}{rgb}{0.199430,0.387607,0.554642}
\definecolor{oceanonefield41}{rgb}{0.195860,0.395433,0.555276}
\definecolor{oceanonefield42}{rgb}{0.192357,0.403199,0.555836}
\definecolor{oceanonefield43}{rgb}{0.188923,0.410910,0.556326}
\definecolor{oceanonefield44}{rgb}{0.185556,0.418570,0.556753}
\definecolor{oceanonefield45}{rgb}{0.182256,0.426184,0.557120}
\definecolor{oceanonefield46}{rgb}{0.179019,0.433756,0.557430}
\definecolor{oceanonefield47}{rgb}{0.175841,0.441290,0.557685}
\definecolor{oceanonefield48}{rgb}{0.172719,0.448791,0.557885}
\definecolor{oceanonefield49}{rgb}{0.169646,0.456262,0.558030}
\definecolor{oceanonefield50}{rgb}{0.166617,0.463708,0.558119}
\definecolor{oceanonefield51}{rgb}{0.163625,0.471133,0.558148}
\definecolor{oceanonefield52}{rgb}{0.160665,0.478540,0.558115}
\definecolor{oceanonefield53}{rgb}{0.157729,0.485932,0.558013}
\definecolor{oceanonefield54}{rgb}{0.154815,0.493313,0.557840}
\definecolor{oceanonefield55}{rgb}{0.151918,0.500685,0.557587}
\definecolor{oceanonefield56}{rgb}{0.149039,0.508051,0.557250}
\definecolor{oceanonefield57}{rgb}{0.146180,0.515413,0.556823}
\definecolor{oceanonefield58}{rgb}{0.143343,0.522773,0.556295}
\definecolor{oceanonefield59}{rgb}{0.140536,0.530132,0.555659}
\definecolor{oceanonefield60}{rgb}{0.137770,0.537492,0.554906}
\definecolor{oceanonefield61}{rgb}{0.135066,0.544853,0.554029}
\definecolor{oceanonefield62}{rgb}{0.132444,0.552216,0.553018}
\definecolor{oceanonefield63}{rgb}{0.129933,0.559582,0.551864}
\definecolor{oceanonefield64}{rgb}{0.126453,0.570633,0.549841}
\definecolor{oceanonefield65}{rgb}{0.124395,0.578002,0.548287}
\definecolor{oceanonefield66}{rgb}{0.122606,0.585371,0.546557}
\definecolor{oceanonefield67}{rgb}{0.121148,0.592739,0.544641}
\definecolor{oceanonefield68}{rgb}{0.120092,0.600104,0.542530}
\definecolor{oceanonefield69}{rgb}{0.119512,0.607464,0.540218}
\definecolor{oceanonefield70}{rgb}{0.119483,0.614817,0.537692}
\definecolor{oceanonefield71}{rgb}{0.120081,0.622161,0.534946}
\definecolor{oceanonefield72}{rgb}{0.121380,0.629492,0.531973}
\definecolor{oceanonefield73}{rgb}{0.123444,0.636809,0.528763}
\definecolor{oceanonefield74}{rgb}{0.126326,0.644107,0.525311}
\definecolor{oceanonefield75}{rgb}{0.130067,0.651384,0.521608}
\definecolor{oceanonefield76}{rgb}{0.134692,0.658636,0.517649}
\definecolor{oceanonefield77}{rgb}{0.140210,0.665859,0.513427}
\definecolor{oceanonefield78}{rgb}{0.146616,0.673050,0.508936}
\definecolor{oceanonefield79}{rgb}{0.153894,0.680203,0.504172}
\definecolor{oceanonefield80}{rgb}{0.162016,0.687316,0.499129}
\definecolor{oceanonefield81}{rgb}{0.170948,0.694384,0.493803}
\definecolor{oceanonefield82}{rgb}{0.180653,0.701402,0.488189}
\definecolor{oceanonefield83}{rgb}{0.191090,0.708366,0.482284}
\definecolor{oceanonefield84}{rgb}{0.202219,0.715272,0.476084}
\definecolor{oceanonefield85}{rgb}{0.214000,0.722114,0.469588}
\definecolor{oceanonefield86}{rgb}{0.226397,0.728888,0.462789}
\definecolor{oceanonefield87}{rgb}{0.239374,0.735588,0.455688}
\definecolor{oceanonefield88}{rgb}{0.252899,0.742211,0.448284}
\definecolor{oceanonefield89}{rgb}{0.266941,0.748751,0.440573}
\definecolor{oceanonefield90}{rgb}{0.281477,0.755203,0.432552}
\definecolor{oceanonefield91}{rgb}{0.296479,0.761561,0.424223}
\definecolor{oceanonefield92}{rgb}{0.311925,0.767822,0.415586}
\definecolor{oceanonefield93}{rgb}{0.327796,0.773980,0.406640}
\definecolor{oceanonefield94}{rgb}{0.344074,0.780029,0.397381}
\definecolor{oceanonefield95}{rgb}{0.360741,0.785964,0.387814}
\definecolor{oceanonefield96}{rgb}{0.377779,0.791781,0.377939}
\definecolor{oceanonefield97}{rgb}{0.395174,0.797475,0.367757}
\definecolor{oceanonefield98}{rgb}{0.412913,0.803041,0.357269}
\definecolor{oceanonefield99}{rgb}{0.430983,0.808473,0.346476}
\definecolor{oceanonefield100}{rgb}{0.449368,0.813768,0.335384}
\definecolor{oceanonefield101}{rgb}{0.468053,0.818921,0.323998}
\definecolor{oceanonefield102}{rgb}{0.487026,0.823929,0.312321}
\definecolor{oceanonefield103}{rgb}{0.506271,0.828786,0.300362}
\definecolor{oceanonefield104}{rgb}{0.525776,0.833491,0.288127}
\definecolor{oceanonefield105}{rgb}{0.545524,0.838039,0.275626}
\definecolor{oceanonefield106}{rgb}{0.565498,0.842430,0.262877}
\definecolor{oceanonefield107}{rgb}{0.585678,0.846661,0.249897}
\definecolor{oceanonefield108}{rgb}{0.606045,0.850733,0.236712}
\definecolor{oceanonefield109}{rgb}{0.626579,0.854645,0.223353}
\definecolor{oceanonefield110}{rgb}{0.647257,0.858400,0.209861}
\definecolor{oceanonefield111}{rgb}{0.668054,0.861999,0.196293}
\definecolor{oceanonefield112}{rgb}{0.688944,0.865448,0.182725}
\definecolor{oceanonefield113}{rgb}{0.709898,0.868751,0.169257}
\definecolor{oceanonefield114}{rgb}{0.730889,0.871916,0.156029}
\definecolor{oceanonefield115}{rgb}{0.751884,0.874951,0.143228}
\definecolor{oceanonefield116}{rgb}{0.772852,0.877868,0.131109}
\definecolor{oceanonefield117}{rgb}{0.793760,0.880678,0.120005}
\definecolor{oceanonefield118}{rgb}{0.814576,0.883393,0.110347}
\definecolor{oceanonefield119}{rgb}{0.835270,0.886029,0.102646}
\definecolor{oceanonefield120}{rgb}{0.855810,0.888601,0.097452}
\definecolor{oceanonefield121}{rgb}{0.876168,0.891125,0.095250}
\definecolor{oceanonefield122}{rgb}{0.896320,0.893616,0.096335}
\definecolor{oceanonefield123}{rgb}{0.916242,0.896091,0.100717}
\definecolor{oceanonefield124}{rgb}{0.935904,0.898570,0.108131}
\definecolor{oceanonefield125}{rgb}{0.955300,0.901065,0.118128}
\definecolor{oceanonefield126}{rgb}{0.974417,0.903590,0.130215}
\definecolor{oceanonefield127}{rgb}{0.993248,0.906157,0.143936}
\definecolor{oceanoneresidual0}{rgb}{0.019608,0.188235,0.380392}
\definecolor{oceanoneresidual1}{rgb}{0.028220,0.204844,0.403460}
\definecolor{oceanoneresidual2}{rgb}{0.036832,0.221453,0.426528}
\definecolor{oceanoneresidual3}{rgb}{0.045444,0.238062,0.449596}
\definecolor{oceanoneresidual4}{rgb}{0.054056,0.254671,0.472664}
\definecolor{oceanoneresidual5}{rgb}{0.062668,0.271280,0.495732}
\definecolor{oceanoneresidual6}{rgb}{0.071280,0.287889,0.518800}
\definecolor{oceanoneresidual7}{rgb}{0.079892,0.304498,0.541869}
\definecolor{oceanoneresidual8}{rgb}{0.088504,0.321107,0.564937}
\definecolor{oceanoneresidual9}{rgb}{0.097116,0.337716,0.588005}
\definecolor{oceanoneresidual10}{rgb}{0.105729,0.354325,0.611073}
\definecolor{oceanoneresidual11}{rgb}{0.114341,0.370934,0.634141}
\definecolor{oceanoneresidual12}{rgb}{0.122953,0.387543,0.657209}
\definecolor{oceanoneresidual13}{rgb}{0.132026,0.403460,0.676278}
\definecolor{oceanoneresidual14}{rgb}{0.142484,0.417301,0.683353}
\definecolor{oceanoneresidual15}{rgb}{0.152941,0.431142,0.690427}
\definecolor{oceanoneresidual16}{rgb}{0.163399,0.444983,0.697501}
\definecolor{oceanoneresidual17}{rgb}{0.173856,0.458824,0.704575}
\definecolor{oceanoneresidual18}{rgb}{0.184314,0.472664,0.711649}
\definecolor{oceanoneresidual19}{rgb}{0.194771,0.486505,0.718724}
\definecolor{oceanoneresidual20}{rgb}{0.205229,0.500346,0.725798}
\definecolor{oceanoneresidual21}{rgb}{0.215686,0.514187,0.732872}
\definecolor{oceanoneresidual22}{rgb}{0.226144,0.528028,0.739946}
\definecolor{oceanoneresidual23}{rgb}{0.236601,0.541869,0.747020}
\definecolor{oceanoneresidual24}{rgb}{0.247059,0.555709,0.754095}
\definecolor{oceanoneresidual25}{rgb}{0.257516,0.569550,0.761169}
\definecolor{oceanoneresidual26}{rgb}{0.274894,0.584160,0.768858}
\definecolor{oceanoneresidual27}{rgb}{0.299193,0.599539,0.777163}
\definecolor{oceanoneresidual28}{rgb}{0.323491,0.614917,0.785467}
\definecolor{oceanoneresidual29}{rgb}{0.347789,0.630296,0.793772}
\definecolor{oceanoneresidual30}{rgb}{0.372088,0.645675,0.802076}
\definecolor{oceanoneresidual31}{rgb}{0.396386,0.661053,0.810381}
\definecolor{oceanoneresidual32}{rgb}{0.420684,0.676432,0.818685}
\definecolor{oceanoneresidual33}{rgb}{0.444983,0.691811,0.826990}
\definecolor{oceanoneresidual34}{rgb}{0.469281,0.707190,0.835294}
\definecolor{oceanoneresidual35}{rgb}{0.493579,0.722568,0.843599}
\definecolor{oceanoneresidual36}{rgb}{0.517878,0.737947,0.851903}
\definecolor{oceanoneresidual37}{rgb}{0.542176,0.753326,0.860208}
\definecolor{oceanoneresidual38}{rgb}{0.566474,0.768704,0.868512}
\definecolor{oceanoneresidual39}{rgb}{0.587082,0.779931,0.874740}
\definecolor{oceanoneresidual40}{rgb}{0.606459,0.789773,0.880277}
\definecolor{oceanoneresidual41}{rgb}{0.625836,0.799616,0.885813}
\definecolor{oceanoneresidual42}{rgb}{0.645213,0.809458,0.891349}
\definecolor{oceanoneresidual43}{rgb}{0.664591,0.819300,0.896886}
\definecolor{oceanoneresidual44}{rgb}{0.683968,0.829143,0.902422}
\definecolor{oceanoneresidual45}{rgb}{0.703345,0.838985,0.907958}
\definecolor{oceanoneresidual46}{rgb}{0.722722,0.848827,0.913495}
\definecolor{oceanoneresidual47}{rgb}{0.742099,0.858670,0.919031}
\definecolor{oceanoneresidual48}{rgb}{0.761476,0.868512,0.924567}
\definecolor{oceanoneresidual49}{rgb}{0.780854,0.878354,0.930104}
\definecolor{oceanoneresidual50}{rgb}{0.800231,0.888197,0.935640}
\definecolor{oceanoneresidual51}{rgb}{0.819608,0.898039,0.941176}
\definecolor{oceanoneresidual52}{rgb}{0.831296,0.903576,0.943329}
\definecolor{oceanoneresidual53}{rgb}{0.842983,0.909112,0.945483}
\definecolor{oceanoneresidual54}{rgb}{0.854671,0.914648,0.947636}
\definecolor{oceanoneresidual55}{rgb}{0.866359,0.920185,0.949789}
\definecolor{oceanoneresidual56}{rgb}{0.878047,0.925721,0.951942}
\definecolor{oceanoneresidual57}{rgb}{0.889735,0.931257,0.954095}
\definecolor{oceanoneresidual58}{rgb}{0.901423,0.936794,0.956248}
\definecolor{oceanoneresidual59}{rgb}{0.913110,0.942330,0.958401}
\definecolor{oceanoneresidual60}{rgb}{0.924798,0.947866,0.960554}
\definecolor{oceanoneresidual61}{rgb}{0.936486,0.953403,0.962707}
\definecolor{oceanoneresidual62}{rgb}{0.948174,0.958939,0.964860}
\definecolor{oceanoneresidual63}{rgb}{0.959862,0.964475,0.967013}
\definecolor{oceanoneresidual64}{rgb}{0.970012,0.962168,0.957555}
\definecolor{oceanoneresidual65}{rgb}{0.971857,0.953556,0.942791}
\definecolor{oceanoneresidual66}{rgb}{0.973702,0.944944,0.928028}
\definecolor{oceanoneresidual67}{rgb}{0.975548,0.936332,0.913264}
\definecolor{oceanoneresidual68}{rgb}{0.977393,0.927720,0.898501}
\definecolor{oceanoneresidual69}{rgb}{0.979239,0.919108,0.883737}
\definecolor{oceanoneresidual70}{rgb}{0.981084,0.910496,0.868973}
\definecolor{oceanoneresidual71}{rgb}{0.982930,0.901884,0.854210}
\definecolor{oceanoneresidual72}{rgb}{0.984775,0.893272,0.839446}
\definecolor{oceanoneresidual73}{rgb}{0.986621,0.884660,0.824683}
\definecolor{oceanoneresidual74}{rgb}{0.988466,0.876048,0.809919}
\definecolor{oceanoneresidual75}{rgb}{0.990311,0.867436,0.795156}
\definecolor{oceanoneresidual76}{rgb}{0.992157,0.858824,0.780392}
\definecolor{oceanoneresidual77}{rgb}{0.989389,0.842215,0.759170}
\definecolor{oceanoneresidual78}{rgb}{0.986621,0.825606,0.737947}
\definecolor{oceanoneresidual79}{rgb}{0.983852,0.808997,0.716724}
\definecolor{oceanoneresidual80}{rgb}{0.981084,0.792388,0.695502}
\definecolor{oceanoneresidual81}{rgb}{0.978316,0.775779,0.674279}
\definecolor{oceanoneresidual82}{rgb}{0.975548,0.759170,0.653057}
\definecolor{oceanoneresidual83}{rgb}{0.972780,0.742561,0.631834}
\definecolor{oceanoneresidual84}{rgb}{0.970012,0.725952,0.610611}
\definecolor{oceanoneresidual85}{rgb}{0.967243,0.709343,0.589389}
\definecolor{oceanoneresidual86}{rgb}{0.964475,0.692734,0.568166}
\definecolor{oceanoneresidual87}{rgb}{0.961707,0.676125,0.546943}
\definecolor{oceanoneresidual88}{rgb}{0.958939,0.659516,0.525721}
\definecolor{oceanoneresidual89}{rgb}{0.954556,0.641753,0.505729}
\definecolor{oceanoneresidual90}{rgb}{0.945329,0.620531,0.489427}
\definecolor{oceanoneresidual91}{rgb}{0.936101,0.599308,0.473126}
\definecolor{oceanoneresidual92}{rgb}{0.926874,0.578085,0.456824}
\definecolor{oceanoneresidual93}{rgb}{0.917647,0.556863,0.440523}
\definecolor{oceanoneresidual94}{rgb}{0.908420,0.535640,0.424221}
\definecolor{oceanoneresidual95}{rgb}{0.899193,0.514418,0.407920}
\definecolor{oceanoneresidual96}{rgb}{0.889965,0.493195,0.391619}
\definecolor{oceanoneresidual97}{rgb}{0.880738,0.471972,0.375317}
\definecolor{oceanoneresidual98}{rgb}{0.871511,0.450750,0.359016}
\definecolor{oceanoneresidual99}{rgb}{0.862284,0.429527,0.342714}
\definecolor{oceanoneresidual100}{rgb}{0.853057,0.408304,0.326413}
\definecolor{oceanoneresidual101}{rgb}{0.843829,0.387082,0.310111}
\definecolor{oceanoneresidual102}{rgb}{0.833679,0.365398,0.296732}
\definecolor{oceanoneresidual103}{rgb}{0.822607,0.343253,0.286275}
\definecolor{oceanoneresidual104}{rgb}{0.811534,0.321107,0.275817}
\definecolor{oceanoneresidual105}{rgb}{0.800461,0.298962,0.265359}
\definecolor{oceanoneresidual106}{rgb}{0.789389,0.276817,0.254902}
\definecolor{oceanoneresidual107}{rgb}{0.778316,0.254671,0.244444}
\definecolor{oceanoneresidual108}{rgb}{0.767243,0.232526,0.233987}
\definecolor{oceanoneresidual109}{rgb}{0.756171,0.210381,0.223529}
\definecolor{oceanoneresidual110}{rgb}{0.745098,0.188235,0.213072}
\definecolor{oceanoneresidual111}{rgb}{0.734025,0.166090,0.202614}
\definecolor{oceanoneresidual112}{rgb}{0.722953,0.143945,0.192157}
\definecolor{oceanoneresidual113}{rgb}{0.711880,0.121799,0.181699}
\definecolor{oceanoneresidual114}{rgb}{0.700807,0.099654,0.171242}
\definecolor{oceanoneresidual115}{rgb}{0.680738,0.088581,0.165859}
\definecolor{oceanoneresidual116}{rgb}{0.657670,0.081200,0.162168}
\definecolor{oceanoneresidual117}{rgb}{0.634602,0.073818,0.158478}
\definecolor{oceanoneresidual118}{rgb}{0.611534,0.066436,0.154787}
\definecolor{oceanoneresidual119}{rgb}{0.588466,0.059054,0.151096}
\definecolor{oceanoneresidual120}{rgb}{0.565398,0.051672,0.147405}
\definecolor{oceanoneresidual121}{rgb}{0.542330,0.044291,0.143714}
\definecolor{oceanoneresidual122}{rgb}{0.519262,0.036909,0.140023}
\definecolor{oceanoneresidual123}{rgb}{0.496194,0.029527,0.136332}
\definecolor{oceanoneresidual124}{rgb}{0.473126,0.022145,0.132641}
\definecolor{oceanoneresidual125}{rgb}{0.450058,0.014764,0.128950}
\definecolor{oceanoneresidual126}{rgb}{0.426990,0.007382,0.125260}
\definecolor{oceanoneresidual127}{rgb}{0.403922,0.000000,0.121569}


==> visualizations/figure1_insert.tex <==
\input{visualizations/figure1_colors.tex}
\newcommand{\RevMainFigure}{%
  \begin{wrapfigure}[21]{R}{0.50\textwidth}
  \centering
  \vspace{-0.9\baselineskip}
  \setlength{\abovecaptionskip}{3pt}
  \input{visualizations/ocean_reference_ours_panel.tex}
  \par\vspace{-0.9\baselineskip}
  \caption{Full-mask ocean reconstructions at $64\times64$, with supplied observations restored in Ours. Black and red outlines mark supplied observations and withheld source-supported scoring locations, respectively. Gray denotes outside-domain locations; white in Reference denotes source-missing values.}
  \label{fig:local-global-reconstruction}
  \end{wrapfigure}%
}


==> visualizations/intro_texture/colorbar.tex <==
\foreach \detailIndex/\detailRed/\detailGreen/\detailBlue in {
0/68/1/84,
1/68/1/84,
2/68/2/86,
3/68/2/86,
4/69/4/87,
5/69/4/87,
6/69/5/89,
7/70/7/90,
8/70/7/90,
9/70/8/92,
10/70/8/92,
11/70/10/93,
12/70/10/93,
13/70/11/94,
14/71/13/96,
15/71/13/96,
16/71/14/97,
17/71/14/97,
18/71/16/99,
19/71/17/100,
20/71/17/100,
21/71/19/101,
22/71/19/101,
23/72/20/103,
24/72/20/103,
25/72/22/104,
26/72/23/105,
27/72/23/105,
28/72/24/106,
29/72/24/106,
30/72/26/108,
31/72/27/109,
32/72/27/109,
33/72/28/110,
34/72/28/110,
35/72/29/111,
36/72/29/111,
37/72/31/112,
38/72/32/113,
39/72/32/113,
40/72/33/115,
41/72/33/115,
42/72/35/116,
43/72/35/116,
44/72/36/117,
45/72/37/118,
46/72/37/118,
47/72/38/119,
48/72/38/119,
49/72/40/120,
50/72/41/121,
51/72/41/121,
52/71/42/122,
53/71/42/122,
54/71/44/122,
55/71/44/122,
56/71/45/123,
57/71/46/124,
58/71/46/124,
59/71/47/125,
60/71/47/125,
61/70/48/126,
62/70/50/126,
63/70/50/126,
64/70/51/127,
65/70/51/127,
66/70/52/128,
67/70/52/128,
68/69/53/129,
69/69/55/129,
70/69/55/129,
71/69/56/130,
72/69/56/130,
73/68/57/131,
74/68/57/131,
75/68/58/131,
76/68/59/132,
77/68/59/132,
78/67/61/132,
79/67/61/132,
80/67/62/133,
81/66/63/133,
82/66/63/133,
83/66/64/134,
84/66/64/134,
85/66/65/134,
86/66/65/134,
87/65/66/135,
88/65/68/135,
89/65/68/135,
90/64/69/136,
91/64/69/136,
92/64/70/136,
93/63/71/136,
94/63/71/136,
95/63/72/137,
96/63/72/137,
97/62/73/137,
98/62/73/137,
99/62/74/137,
100/62/76/138,
101/62/76/138,
102/61/77/138,
103/61/77/138,
104/61/78/138,
105/61/78/138,
106/60/79/138,
107/60/80/139,
108/60/80/139,
109/59/81/139,
110/59/81/139,
111/59/82/139,
112/58/83/139,
113/58/83/139,
114/58/84/140,
115/58/84/140,
116/57/85/140,
117/57/85/140,
118/57/86/140,
119/56/88/140,
120/56/88/140,
121/56/89/140,
122/56/89/140,
123/55/90/140,
124/55/91/141,
125/55/91/141,
126/54/92/141,
127/54/92/141,
128/54/93/141,
129/54/93/141,
130/53/94/141,
131/53/95/141,
132/53/95/141,
133/52/96/141,
134/52/96/141,
135/52/97/141,
136/52/97/141,
137/51/98/141,
138/51/99/141,
139/51/99/141,
140/50/100/142,
141/50/100/142,
142/50/101/142,
143/49/102/142,
144/49/102/142,
145/49/103/142,
146/49/103/142,
147/49/104/142,
148/49/104/142,
149/48/105/142,
150/48/106/142,
151/48/106/142,
152/47/107/142,
153/47/107/142,
154/47/108/142,
155/46/109/142,
156/46/109/142,
157/46/110/142,
158/46/110/142,
159/46/111/142,
160/46/111/142,
161/45/112/142,
162/45/113/142,
163/45/113/142,
164/44/113/142,
165/44/113/142,
166/44/114/142,
167/44/114/142,
168/44/115/142,
169/43/116/142,
170/43/116/142,
171/43/117/142,
172/43/117/142,
173/42/118/142,
174/42/119/142,
175/42/119/142,
176/42/120/142,
177/42/120/142,
178/41/121/142,
179/41/121/142,
180/41/122/142,
181/41/123/142,
182/41/123/142,
183/40/124/142,
184/40/124/142,
185/40/125/142,
186/39/126/142,
187/39/126/142,
188/39/127/142,
189/39/127/142,
190/39/128/142,
191/39/128/142,
192/38/129/142,
193/38/130/142,
194/38/130/142,
195/38/130/142,
196/38/130/142,
197/37/131/142,
198/37/131/142,
199/37/132/142,
200/37/133/142,
201/37/133/142,
202/36/134/142,
203/36/134/142,
204/36/135/142,
205/35/136/142,
206/35/136/142,
207/35/137/142,
208/35/137/142,
209/35/138/141,
210/35/138/141,
211/34/139/141,
212/34/140/141,
213/34/140/141,
214/34/141/141,
215/34/141/141,
216/33/142/141,
217/33/143/141,
218/33/143/141,
219/33/144/141,
220/33/144/141,
221/33/145/140,
222/33/145/140,
223/32/146/140,
224/32/146/140,
225/32/146/140,
226/32/147/140,
227/32/147/140,
228/31/148/140,
229/31/148/140,
230/31/149/139,
231/31/150/139,
232/31/150/139,
233/31/151/139,
234/31/151/139,
235/31/152/139,
236/31/153/138,
237/31/153/138,
238/31/154/138,
239/31/154/138,
240/30/155/138,
241/30/155/138,
242/30/156/137,
243/30/157/137,
244/30/157/137,
245/31/158/137,
246/31/158/137,
247/31/159/136,
248/31/160/136,
249/31/160/136,
250/31/161/136,
251/31/161/136,
252/31/161/135,
253/31/161/135,
254/31/162/135,
255/32/163/134,
256/32/163/134,
257/32/164/134,
258/32/164/134,
259/33/165/133,
260/33/165/133,
261/33/166/133,
262/34/167/133,
263/34/167/133,
264/34/168/132,
265/34/168/132,
266/35/169/131,
267/36/170/131,
268/36/170/131,
269/37/171/130,
270/37/171/130,
271/37/172/130,
272/37/172/130,
273/38/173/129,
274/39/173/129,
275/39/173/129,
276/40/174/128,
277/40/174/128,
278/41/175/127,
279/42/176/127,
280/42/176/127,
281/44/177/126,
282/44/177/126,
283/45/178/125,
284/45/178/125,
285/46/179/124,
286/47/180/124,
287/47/180/124,
288/49/181/123,
289/49/181/123,
290/50/182/122,
291/50/182/122,
292/52/182/121,
293/53/183/121,
294/53/183/121,
295/55/184/120,
296/55/184/120,
297/56/185/119,
298/58/186/118,
299/58/186/118,
300/59/187/117,
301/59/187/117,
302/61/188/116,
303/61/188/116,
304/63/188/115,
305/64/189/114,
306/64/189/114,
307/66/190/113,
308/66/190/113,
309/68/191/112,
310/68/191/112,
311/70/192/111,
312/72/193/110,
313/72/193/110,
314/74/193/109,
315/74/193/109,
316/76/194/108,
317/78/195/107,
318/78/195/107,
319/80/196/106,
320/80/196/106,
321/82/197/105,
322/82/197/105,
323/84/197/104,
324/86/198/103,
325/86/198/103,
326/88/199/101,
327/88/199/101,
328/90/200/100,
329/92/200/99,
330/92/200/99,
331/94/201/98,
332/94/201/98,
333/96/202/96,
334/96/202/96,
335/99/203/95,
336/101/203/94,
337/101/203/94,
338/103/204/92,
339/103/204/92,
340/105/205/91,
341/105/205/91,
342/108/205/90,
343/110/206/88,
344/110/206/88,
345/112/207/87,
346/112/207/87,
347/115/208/86,
348/117/208/84,
349/117/208/84,
350/119/209/83,
351/119/209/83,
352/122/209/81,
353/122/209/81,
354/124/210/80,
355/127/211/78,
356/127/211/78,
357/129/211/77,
358/129/211/77,
359/132/212/75,
360/134/213/73,
361/134/213/73,
362/137/213/72,
363/137/213/72,
364/139/214/70,
365/139/214/70,
366/142/214/69,
367/144/215/67,
368/144/215/67,
369/147/215/65,
370/147/215/65,
371/149/216/64,
372/149/216/64,
373/152/216/62,
374/155/217/60,
375/155/217/60,
376/157/217/59,
377/157/217/59,
378/160/218/57,
379/162/218/55,
380/162/218/55,
381/165/219/54,
382/165/219/54,
383/168/219/52,
384/168/219/52,
385/170/220/50,
386/173/220/48,
387/173/220/48,
388/176/221/47,
389/176/221/47,
390/178/221/45,
391/181/222/43,
392/181/222/43,
393/184/222/41,
394/184/222/41,
395/186/222/40,
396/186/222/40,
397/189/223/38,
398/192/223/37,
399/192/223/37,
400/194/223/35,
401/194/223/35,
402/197/224/33,
403/197/224/33,
404/200/224/32,
405/202/225/31,
406/202/225/31,
407/205/225/29,
408/205/225/29,
409/208/225/28,
410/210/226/27,
411/210/226/27,
412/213/226/26,
413/213/226/26,
414/216/226/25,
415/216/226/25,
416/218/227/25,
417/221/227/24,
418/221/227/24,
419/223/227/24,
420/223/227/24,
421/226/228/24,
422/229/228/25,
423/229/228/25,
424/231/228/25,
425/231/228/25,
426/234/229/26,
427/234/229/26,
428/236/229/27,
429/239/229/28,
430/239/229/28,
431/241/229/29,
432/241/229/29,
433/244/230/30,
434/244/230/30,
435/246/230/32,
436/248/230/33,
437/248/230/33,
438/251/231/35,
439/251/231/35,
440/253/231/37
} {
  \definecolor{detailBarColor}{RGB}{\detailRed,\detailGreen,\detailBlue}
  \path[fill=detailBarColor,draw=none] ({\DetailBarX+\DetailBarWidth*\detailIndex/441},33.15) rectangle ({\DetailBarX+\DetailBarWidth*(\detailIndex+1)/441},34.55);
}
\node[anchor=base,font=\fontsize{10}{11}\selectfont] at (\DetailBarX,37.55) {$-1$};
\node[anchor=base,font=\fontsize{10}{11}\selectfont] at ({\DetailBarX+\DetailBarWidth/2},37.55) {$0$};
\node[anchor=base,font=\fontsize{10}{11}\selectfont] at ({\DetailBarX+\DetailBarWidth},37.55) {$1$};


==> visualizations/ns_texture/colorbar.tex <==
\foreach \detailIndex/\detailRed/\detailGreen/\detailBlue in {
0/5/48/97,
1/6/50/100,
2/6/50/100,
3/7/52/103,
4/8/54/106,
5/9/56/109,
6/10/59/112,
7/12/61/115,
8/12/61/115,
9/13/63/118,
10/14/65/121,
11/15/67/123,
12/16/69/126,
13/16/69/126,
14/17/71/129,
15/18/73/132,
16/19/76/135,
17/20/78/138,
18/20/78/138,
19/21/80/141,
20/23/82/144,
21/24/84/147,
22/25/86/150,
23/26/88/153,
24/26/88/153,
25/27/90/156,
26/28/92/159,
27/29/95/162,
28/30/97/165,
29/30/97/165,
30/31/99/168,
31/32/101/171,
32/34/103/172,
33/35/105/173,
34/36/106/174,
35/36/106/174,
36/38/108/175,
37/39/110/176,
38/40/112/177,
39/42/113/178,
40/42/113/178,
41/43/115/179,
42/44/117/180,
43/46/119/181,
44/47/121/181,
45/47/121/181,
46/48/122/182,
47/50/124/183,
48/51/126/184,
49/52/128/185,
50/54/129/186,
51/54/129/186,
52/55/131/187,
53/56/133/188,
54/58/135/189,
55/59/136/190,
56/59/136/190,
57/60/138/190,
58/62/140/191,
59/63/142/192,
60/64/143/193,
61/64/143/193,
62/66/145/194,
63/67/147/195,
64/70/149/196,
65/73/151/197,
66/76/153/198,
67/76/153/198,
68/79/155/199,
69/82/157/200,
70/86/159/201,
71/89/161/202,
72/89/161/202,
73/92/163/203,
74/95/165/205,
75/98/167/206,
76/101/169/207,
77/101/169/207,
78/104/171/208,
79/107/172/209,
80/110/174/210,
81/113/176/211,
82/117/178/212,
83/117/178/212,
84/120/180/213,
85/123/182/214,
86/126/184/215,
87/129/186/216,
88/129/186/216,
89/132/188/217,
90/135/190/218,
91/138/192/219,
92/141/194/220,
93/141/194/220,
94/144/196/221,
95/147/198/222,
96/150/199/223,
97/152/200/224,
98/155/201/224,
99/155/201/224,
100/157/203/225,
101/160/204/226,
102/162/205/227,
103/165/206/227,
104/165/206/227,
105/167/208/228,
106/169/209/229,
107/172/210/229,
108/174/211/230,
109/174/211/230,
110/177/213/231,
111/179/214/232,
112/182/215/232,
113/184/216/233,
114/187/218/234,
115/187/218/234,
116/189/219/234,
117/192/220/235,
118/194/221/236,
119/197/223/236,
120/197/223/236,
121/199/224/237,
122/202/225/238,
123/204/226/239,
124/207/228/239,
125/207/228/239,
126/209/229/240,
127/210/230/240,
128/212/230/241,
129/213/231/241,
130/215/232/241,
131/215/232/241,
132/216/233/241,
133/218/233/242,
134/219/234/242,
135/221/235/242,
136/221/235/242,
137/222/235/242,
138/224/236/243,
139/225/237/243,
140/227/237/243,
141/227/237/243,
142/228/238/244,
143/230/239/244,
144/231/240/244,
145/233/240/244,
146/234/241/245,
147/234/241/245,
148/236/242/245,
149/237/242/245,
150/239/243/245,
151/240/244/246,
152/240/244/246,
153/242/245/246,
154/243/245/246,
155/245/246/247,
156/246/247/247,
157/246/247/247,
158/247/246/246,
159/247/245/244,
160/248/244/242,
161/248/243/240,
162/248/242/239,
163/248/242/239,
164/248/241/237,
165/249/240/235,
166/249/239/233,
167/249/238/231,
168/249/238/231,
169/249/237/229,
170/249/235/227,
171/250/234/225,
172/250/233/223,
173/250/233/223,
174/250/232/222,
175/250/231/220,
176/251/230/218,
177/251/229/216,
178/251/228/214,
179/251/228/214,
180/251/227/212,
181/252/226/210,
182/252/224/208,
183/252/223/207,
184/252/223/207,
185/252/222/205,
186/253/221/203,
187/253/220/201,
188/253/219/199,
189/253/219/199,
190/253/217/196,
191/252/215/194,
192/252/213/191,
193/252/211/188,
194/251/208/185,
195/251/208/185,
196/251/206/183,
197/251/204/180,
198/250/202/177,
199/250/200/175,
200/250/200/175,
201/249/198/172,
202/249/196/169,
203/249/194/167,
204/248/191/164,
205/248/191/164,
206/248/189/161,
207/248/187/158,
208/247/185/156,
209/247/183/153,
210/247/181/150,
211/247/181/150,
212/246/179/148,
213/246/177/145,
214/246/175/142,
215/245/172/139,
216/245/172/139,
217/245/170/137,
218/245/168/134,
219/244/166/131,
220/243/164/129,
221/243/164/129,
222/242/161/127,
223/241/158/125,
224/240/156/123,
225/239/153/121,
226/238/150/119,
227/238/150/119,
228/236/147/116,
229/235/145/114,
230/234/142/112,
231/233/139/110,
232/233/139/110,
233/232/137/108,
234/230/134/106,
235/229/131/104,
236/228/128/102,
237/227/126/100,
238/227/126/100,
239/226/123/98,
240/225/120/96,
241/223/118/94,
242/222/115/92,
243/222/115/92,
244/221/112/89,
245/220/110/87,
246/219/107/85,
247/218/104/83,
248/218/104/83,
249/216/101/81,
250/215/99/79,
251/214/96/77,
252/213/93/76,
253/211/90/74,
254/211/90/74,
255/210/88/73,
256/208/85/72,
257/207/82/70,
258/206/79/69,
259/206/79/69,
260/204/76/68,
261/203/73/66,
262/201/71/65,
263/200/68/64,
264/200/68/64,
265/198/65/62,
266/197/62/61,
267/196/59/60,
268/194/56/58,
269/193/54/57,
270/193/54/57,
271/191/51/56,
272/190/48/54,
273/189/45/53,
274/187/42/52,
275/187/42/52,
276/186/40/50,
277/184/37/49,
278/183/34/48,
279/182/31/46,
280/182/31/46,
281/180/28/45,
282/179/25/44,
283/177/24/43,
284/174/23/42,
285/171/22/42,
286/171/22/42,
287/168/21/41,
288/165/20/41,
289/162/19/40,
290/159/18/40,
291/159/18/40,
292/156/17/39,
293/153/16/39,
294/150/15/39,
295/147/14/38,
296/147/14/38,
297/144/13/38,
298/141/12/37,
299/138/11/37,
300/135/10/36,
301/132/9/36,
302/132/9/36,
303/129/8/35,
304/127/8/35,
305/124/7/34,
306/121/6/34,
307/121/6/34,
308/118/5/33,
309/115/4/33,
310/112/3/32,
311/109/2/32,
312/109/2/32,
313/106/1/31,
314/103/0/31
} {
  \definecolor{detailBarColor}{RGB}{\detailRed,\detailGreen,\detailBlue}
  \path[fill=detailBarColor,draw=none] ({\DetailBarX+\DetailBarWidth*\detailIndex/315},33.15) rectangle ({\DetailBarX+\DetailBarWidth*(\detailIndex+1)/315},34.55);
}
\node[anchor=base,font=\fontsize{10}{11}\selectfont] at (\DetailBarX,37.55) {$-1$};
\node[anchor=base,font=\fontsize{10}{11}\selectfont] at ({\DetailBarX+\DetailBarWidth/2},37.55) {$0$};
\node[anchor=base,font=\fontsize{10}{11}\selectfont] at ({\DetailBarX+\DetailBarWidth},37.55) {$1$};


==> visualizations/ocean_selected_figures.tex <==
\input{visualizations/ocean_selected_task2_colors.tex}
\newcommand{\RevOceanFigure}{%
  \input{visualizations/ocean_selected_task2_chl.tex}%
  \input{visualizations/ocean_selected_task2_nano.tex}%
  \input{visualizations/ocean_selected_task2_sss.tex}%
}
\newcommand{\RevOceanHighResolutionFigure}{%
  \input{visualizations/ocean_selected_task3_chl.tex}%
  \input{visualizations/ocean_selected_task3_nano.tex}%
  \input{visualizations/ocean_selected_task3_sss.tex}%
}


==> visualizations/ocean_selected_task2_colors.tex <==
\definecolor{oceantwofield0}{rgb}{0.267004,0.004874,0.329415}
\definecolor{oceantwofield1}{rgb}{0.269944,0.014625,0.341379}
\definecolor{oceantwofield2}{rgb}{0.272594,0.025563,0.353093}
\definecolor{oceantwofield3}{rgb}{0.274952,0.037752,0.364543}
\definecolor{oceantwofield4}{rgb}{0.277018,0.050344,0.375715}
\definecolor{oceantwofield5}{rgb}{0.278791,0.062145,0.386592}
\definecolor{oceantwofield6}{rgb}{0.280267,0.073417,0.397163}
\definecolor{oceantwofield7}{rgb}{0.281446,0.084320,0.407414}
\definecolor{oceantwofield8}{rgb}{0.282327,0.094955,0.417331}
\definecolor{oceantwofield9}{rgb}{0.282910,0.105393,0.426902}
\definecolor{oceantwofield10}{rgb}{0.283197,0.115680,0.436115}
\definecolor{oceantwofield11}{rgb}{0.283187,0.125848,0.444960}
\definecolor{oceantwofield12}{rgb}{0.282884,0.135920,0.453427}
\definecolor{oceantwofield13}{rgb}{0.282290,0.145912,0.461510}
\definecolor{oceantwofield14}{rgb}{0.281412,0.155834,0.469201}
\definecolor{oceantwofield15}{rgb}{0.280255,0.165693,0.476498}
\definecolor{oceantwofield16}{rgb}{0.278826,0.175490,0.483397}
\definecolor{oceantwofield17}{rgb}{0.277134,0.185228,0.489898}
\definecolor{oceantwofield18}{rgb}{0.275191,0.194905,0.496005}
\definecolor{oceantwofield19}{rgb}{0.273006,0.204520,0.501721}
\definecolor{oceantwofield20}{rgb}{0.270595,0.214069,0.507052}
\definecolor{oceantwofield21}{rgb}{0.267968,0.223549,0.512008}
\definecolor{oceantwofield22}{rgb}{0.265145,0.232956,0.516599}
\definecolor{oceantwofield23}{rgb}{0.262138,0.242286,0.520837}
\definecolor{oceantwofield24}{rgb}{0.258965,0.251537,0.524736}
\definecolor{oceantwofield25}{rgb}{0.255645,0.260703,0.528312}
\definecolor{oceantwofield26}{rgb}{0.252194,0.269783,0.531579}
\definecolor{oceantwofield27}{rgb}{0.248629,0.278775,0.534556}
\definecolor{oceantwofield28}{rgb}{0.244972,0.287675,0.537260}
\definecolor{oceantwofield29}{rgb}{0.241237,0.296485,0.539709}
\definecolor{oceantwofield30}{rgb}{0.237441,0.305202,0.541921}
\definecolor{oceantwofield31}{rgb}{0.233603,0.313828,0.543914}
\definecolor{oceantwofield32}{rgb}{0.229739,0.322361,0.545706}
\definecolor{oceantwofield33}{rgb}{0.225863,0.330805,0.547314}
\definecolor{oceantwofield34}{rgb}{0.221989,0.339161,0.548752}
\definecolor{oceantwofield35}{rgb}{0.218130,0.347432,0.550038}
\definecolor{oceantwofield36}{rgb}{0.214298,0.355619,0.551184}
\definecolor{oceantwofield37}{rgb}{0.210503,0.363727,0.552206}
\definecolor{oceantwofield38}{rgb}{0.206756,0.371758,0.553117}
\definecolor{oceantwofield39}{rgb}{0.203063,0.379716,0.553925}
\definecolor{oceantwofield40}{rgb}{0.199430,0.387607,0.554642}
\definecolor{oceantwofield41}{rgb}{0.195860,0.395433,0.555276}
\definecolor{oceantwofield42}{rgb}{0.192357,0.403199,0.555836}
\definecolor{oceantwofield43}{rgb}{0.188923,0.410910,0.556326}
\definecolor{oceantwofield44}{rgb}{0.185556,0.418570,0.556753}
\definecolor{oceantwofield45}{rgb}{0.182256,0.426184,0.557120}
\definecolor{oceantwofield46}{rgb}{0.179019,0.433756,0.557430}
\definecolor{oceantwofield47}{rgb}{0.175841,0.441290,0.557685}
\definecolor{oceantwofield48}{rgb}{0.172719,0.448791,0.557885}
\definecolor{oceantwofield49}{rgb}{0.169646,0.456262,0.558030}
\definecolor{oceantwofield50}{rgb}{0.166617,0.463708,0.558119}
\definecolor{oceantwofield51}{rgb}{0.163625,0.471133,0.558148}
\definecolor{oceantwofield52}{rgb}{0.160665,0.478540,0.558115}
\definecolor{oceantwofield53}{rgb}{0.157729,0.485932,0.558013}
\definecolor{oceantwofield54}{rgb}{0.154815,0.493313,0.557840}
\definecolor{oceantwofield55}{rgb}{0.151918,0.500685,0.557587}
\definecolor{oceantwofield56}{rgb}{0.149039,0.508051,0.557250}
\definecolor{oceantwofield57}{rgb}{0.146180,0.515413,0.556823}
\definecolor{oceantwofield58}{rgb}{0.143343,0.522773,0.556295}
\definecolor{oceantwofield59}{rgb}{0.140536,0.530132,0.555659}
\definecolor{oceantwofield60}{rgb}{0.137770,0.537492,0.554906}
\definecolor{oceantwofield61}{rgb}{0.135066,0.544853,0.554029}
\definecolor{oceantwofield62}{rgb}{0.132444,0.552216,0.553018}
\definecolor{oceantwofield63}{rgb}{0.129933,0.559582,0.551864}
\definecolor{oceantwofield64}{rgb}{0.126453,0.570633,0.549841}
\definecolor{oceantwofield65}{rgb}{0.124395,0.578002,0.548287}
\definecolor{oceantwofield66}{rgb}{0.122606,0.585371,0.546557}
\definecolor{oceantwofield67}{rgb}{0.121148,0.592739,0.544641}
\definecolor{oceantwofield68}{rgb}{0.120092,0.600104,0.542530}
\definecolor{oceantwofield69}{rgb}{0.119512,0.607464,0.540218}
\definecolor{oceantwofield70}{rgb}{0.119483,0.614817,0.537692}
\definecolor{oceantwofield71}{rgb}{0.120081,0.622161,0.534946}
\definecolor{oceantwofield72}{rgb}{0.121380,0.629492,0.531973}
\definecolor{oceantwofield73}{rgb}{0.123444,0.636809,0.528763}
\definecolor{oceantwofield74}{rgb}{0.126326,0.644107,0.525311}
\definecolor{oceantwofield75}{rgb}{0.130067,0.651384,0.521608}
\definecolor{oceantwofield76}{rgb}{0.134692,0.658636,0.517649}
\definecolor{oceantwofield77}{rgb}{0.140210,0.665859,0.513427}
\definecolor{oceantwofield78}{rgb}{0.146616,0.673050,0.508936}
\definecolor{oceantwofield79}{rgb}{0.153894,0.680203,0.504172}
\definecolor{oceantwofield80}{rgb}{0.162016,0.687316,0.499129}
\definecolor{oceantwofield81}{rgb}{0.170948,0.694384,0.493803}
\definecolor{oceantwofield82}{rgb}{0.180653,0.701402,0.488189}
\definecolor{oceantwofield83}{rgb}{0.191090,0.708366,0.482284}
\definecolor{oceantwofield84}{rgb}{0.202219,0.715272,0.476084}
\definecolor{oceantwofield85}{rgb}{0.214000,0.722114,0.469588}
\definecolor{oceantwofield86}{rgb}{0.226397,0.728888,0.462789}
\definecolor{oceantwofield87}{rgb}{0.239374,0.735588,0.455688}
\definecolor{oceantwofield88}{rgb}{0.252899,0.742211,0.448284}
\definecolor{oceantwofield89}{rgb}{0.266941,0.748751,0.440573}
\definecolor{oceantwofield90}{rgb}{0.281477,0.755203,0.432552}
\definecolor{oceantwofield91}{rgb}{0.296479,0.761561,0.424223}
\definecolor{oceantwofield92}{rgb}{0.311925,0.767822,0.415586}
\definecolor{oceantwofield93}{rgb}{0.327796,0.773980,0.406640}
\definecolor{oceantwofield94}{rgb}{0.344074,0.780029,0.397381}
\definecolor{oceantwofield95}{rgb}{0.360741,0.785964,0.387814}
\definecolor{oceantwofield96}{rgb}{0.377779,0.791781,0.377939}
\definecolor{oceantwofield97}{rgb}{0.395174,0.797475,0.367757}
\definecolor{oceantwofield98}{rgb}{0.412913,0.803041,0.357269}
\definecolor{oceantwofield99}{rgb}{0.430983,0.808473,0.346476}
\definecolor{oceantwofield100}{rgb}{0.449368,0.813768,0.335384}
\definecolor{oceantwofield101}{rgb}{0.468053,0.818921,0.323998}
\definecolor{oceantwofield102}{rgb}{0.487026,0.823929,0.312321}
\definecolor{oceantwofield103}{rgb}{0.506271,0.828786,0.300362}
\definecolor{oceantwofield104}{rgb}{0.525776,0.833491,0.288127}
\definecolor{oceantwofield105}{rgb}{0.545524,0.838039,0.275626}
\definecolor{oceantwofield106}{rgb}{0.565498,0.842430,0.262877}
\definecolor{oceantwofield107}{rgb}{0.585678,0.846661,0.249897}
\definecolor{oceantwofield108}{rgb}{0.606045,0.850733,0.236712}
\definecolor{oceantwofield109}{rgb}{0.626579,0.854645,0.223353}
\definecolor{oceantwofield110}{rgb}{0.647257,0.858400,0.209861}
\definecolor{oceantwofield111}{rgb}{0.668054,0.861999,0.196293}
\definecolor{oceantwofield112}{rgb}{0.688944,0.865448,0.182725}
\definecolor{oceantwofield113}{rgb}{0.709898,0.868751,0.169257}
\definecolor{oceantwofield114}{rgb}{0.730889,0.871916,0.156029}
\definecolor{oceantwofield115}{rgb}{0.751884,0.874951,0.143228}
\definecolor{oceantwofield116}{rgb}{0.772852,0.877868,0.131109}
\definecolor{oceantwofield117}{rgb}{0.793760,0.880678,0.120005}
\definecolor{oceantwofield118}{rgb}{0.814576,0.883393,0.110347}
\definecolor{oceantwofield119}{rgb}{0.835270,0.886029,0.102646}
\definecolor{oceantwofield120}{rgb}{0.855810,0.888601,0.097452}
\definecolor{oceantwofield121}{rgb}{0.876168,0.891125,0.095250}
\definecolor{oceantwofield122}{rgb}{0.896320,0.893616,0.096335}
\definecolor{oceantwofield123}{rgb}{0.916242,0.896091,0.100717}
\definecolor{oceantwofield124}{rgb}{0.935904,0.898570,0.108131}
\definecolor{oceantwofield125}{rgb}{0.955300,0.901065,0.118128}
\definecolor{oceantwofield126}{rgb}{0.974417,0.903590,0.130215}
\definecolor{oceantwofield127}{rgb}{0.993248,0.906157,0.143936}


==> visualizations/setup.tex <==
\RequirePackage{graphicx}
\RequirePackage{xcolor}
\RequirePackage{array}
\RequirePackage{tikz}
\RequirePackage{wrapfig}
\RequirePackage{placeins}

\newcommand{\VisualizationLabelFont}{\fontsize{11.6}{12.5}\selectfont}
\setcounter{topnumber}{6}
\setcounter{bottomnumber}{6}
\setcounter{totalnumber}{8}
\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{10pt plus 2pt minus 2pt}
\setlength{\@fpbot}{0pt plus 1fil}
\makeatother

\input{visualizations/figure1_insert.tex}
\input{visualizations/ocean_selected_figures.tex}

